FC-GAGA: Fully Connected Gated Graph Architecture for Spatio-Temporal Traffic Forecasting

Forecasting of multivariate time-series is an important problem that has applications in traffic management, cellular network configuration, and quantitative finance. A special case of the problem arises when there is a graph available that captures the relationships between the time-series. In this paper we propose a novel learning architecture that achieves performance competitive with or better than the best existing algorithms, without requiring knowledge of the graph. The key element of our proposed architecture is the learnable fully connected hard graph gating mechanism that enables the use of the state-of-the-art and highly computationally efficient fully connected time-series forecasting architecture in traffic forecasting applications. Experimental results for two public traffic network datasets illustrate the value of our approach, and ablation studies confirm the importance of each element of the architecture. The code is available here: https://github.com/boreshkinai/fc-gaga.

==> results/metr-la-3layers.tex <==
Early stop test error model repeat=0;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 3.057
Horizon 3 MAE: 2.74 Horizon 3 MAPE: 7.2 Horizon 3 RMSE: 5.31
Horizon 6 MAE: 3.09 Horizon 6 MAPE: 8.55 Horizon 6 RMSE: 6.28
Horizon 9 MAE: 3.34 Horizon 9 MAPE: 9.55 Horizon 9 RMSE: 6.91
Horizon 12 MAE: 3.51 Horizon 12 MAPE: 10.21 Horizon 12 RMSE: 7.3
Early stop test error model repeat=1;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 3.061
Horizon 3 MAE: 2.76 Horizon 3 MAPE: 7.26 Horizon 3 RMSE: 5.33
Horizon 6 MAE: 3.1 Horizon 6 MAPE: 8.59 Horizon 6 RMSE: 6.29
Horizon 9 MAE: 3.33 Horizon 9 MAPE: 9.46 Horizon 9 RMSE: 6.88
Horizon 12 MAE: 3.49 Horizon 12 MAPE: 10.11 Horizon 12 RMSE: 7.26
Early stop test error model repeat=2;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 3.07
Horizon 3 MAE: 2.76 Horizon 3 MAPE: 7.32 Horizon 3 RMSE: 5.37
Horizon 6 MAE: 3.11 Horizon 6 MAPE: 8.6 Horizon 6 RMSE: 6.33
Horizon 9 MAE: 3.33 Horizon 9 MAPE: 9.43 Horizon 9 RMSE: 6.91
Horizon 12 MAE: 3.51 Horizon 12 MAPE: 10.03 Horizon 12 RMSE: 7.3
Early stop test error model repeat=3;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 3.077
Horizon 3 MAE: 2.76 Horizon 3 MAPE: 7.22 Horizon 3 RMSE: 5.33
Horizon 6 MAE: 3.12 Horizon 6 MAPE: 8.53 Horizon 6 RMSE: 6.3
Horizon 9 MAE: 3.35 Horizon 9 MAPE: 9.47 Horizon 9 RMSE: 6.89
Horizon 12 MAE: 3.54 Horizon 12 MAPE: 10.18 Horizon 12 RMSE: 7.36
Early stop test error model repeat=4;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 3.067
Horizon 3 MAE: 2.75 Horizon 3 MAPE: 7.27 Horizon 3 RMSE: 5.35
Horizon 6 MAE: 3.1 Horizon 6 MAPE: 8.57 Horizon 6 RMSE: 6.3
Horizon 9 MAE: 3.33 Horizon 9 MAPE: 9.42 Horizon 9 RMSE: 6.88
Horizon 12 MAE: 3.52 Horizon 12 MAPE: 10.16 Horizon 12 RMSE: 7.31

Average MAE: {3: 2.75, 6: 3.1, 9: 3.33, 12: 3.51}
Average MAPE: {3: 7.25, 6: 8.57, 9: 9.47, 12: 10.14}
Average RMSE: {3: 5.34, 6: 6.3, 9: 6.9, 12: 7.31}

==> results/pems-bay-3layer.tex <==
Early stop test error model repeat=0;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 1.628
Horizon 3 MAE: 1.36 Horizon 3 MAPE: 2.88 Horizon 3 RMSE: 2.86
Horizon 6 MAE: 1.69 Horizon 6 MAPE: 3.85 Horizon 6 RMSE: 3.82
Horizon 9 MAE: 1.88 Horizon 9 MAPE: 4.43 Horizon 9 RMSE: 4.29
Horizon 12 MAE: 1.99 Horizon 12 MAPE: 4.77 Horizon 12 RMSE: 4.58
Early stop test error model repeat=1;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 1.62
Horizon 3 MAE: 1.38 Horizon 3 MAPE: 2.91 Horizon 3 RMSE: 2.89
Horizon 6 MAE: 1.68 Horizon 6 MAPE: 3.81 Horizon 6 RMSE: 3.8
Horizon 9 MAE: 1.85 Horizon 9 MAPE: 4.37 Horizon 9 RMSE: 4.26
Horizon 12 MAE: 1.97 Horizon 12 MAPE: 4.72 Horizon 12 RMSE: 4.52
Early stop test error model repeat=2;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 1.612
Horizon 3 MAE: 1.36 Horizon 3 MAPE: 2.86 Horizon 3 RMSE: 2.84
Horizon 6 MAE: 1.68 Horizon 6 MAPE: 3.8 Horizon 6 RMSE: 3.78
Horizon 9 MAE: 1.84 Horizon 9 MAPE: 4.28 Horizon 9 RMSE: 4.22
Horizon 12 MAE: 1.97 Horizon 12 MAPE: 4.64 Horizon 12 RMSE: 4.51
Early stop test error model repeat=3;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 1.601
Horizon 3 MAE: 1.35 Horizon 3 MAPE: 2.83 Horizon 3 RMSE: 2.85
Horizon 6 MAE: 1.67 Horizon 6 MAPE: 3.71 Horizon 6 RMSE: 3.77
Horizon 9 MAE: 1.83 Horizon 9 MAPE: 4.21 Horizon 9 RMSE: 4.19
Horizon 12 MAE: 1.95 Horizon 12 MAPE: 4.54 Horizon 12 RMSE: 4.45
Early stop test error model repeat=4;epochs=60;steps_per_epoch=800;block_layers=3;blocks=2;weight_decay=1e-05;num_stacks=3;epsilon=10: Avg MAE 1.62
Horizon 3 MAE: 1.36 Horizon 3 MAPE: 2.87 Horizon 3 RMSE: 2.85
Horizon 6 MAE: 1.69 Horizon 6 MAPE: 3.83 Horizon 6 RMSE: 3.81
Horizon 9 MAE: 1.85 Horizon 9 MAPE: 4.34 Horizon 9 RMSE: 4.25
Horizon 12 MAE: 1.97 Horizon 12 MAPE: 4.68 Horizon 12 RMSE: 4.5

Average MAE: {3: 1.36, 6: 1.68, 9: 1.85, 12: 1.97}
Average MAPE: {3: 2.87, 6: 3.8, 9: 4.32, 12: 4.67}
Average RMSE: {3: 2.86, 6: 3.8, 9: 4.24, 12: 4.52}
